4D Feet: Registering Walking Foot Shapes Using Attention Enhanced Dynamic-Synchronized Graph Convolutional LSTM Network

4D scans of dynamic deformable human body parts help researchers have a better understanding of spatiotemporal features. However, reconstructing 4D scans based on multiple asynchronous cameras encounters two main challenges: 1) finding the dynamic correspondences among different frames captured by each camera at the timestamps of the camera in terms of dynamic feature recognition, and 2) reconstructing 3D shapes from the combined point clouds captured by different cameras at asynchronous timestamps in terms of multi-view fusion. In this paper, we introduce a generic framework that is able to 1) find and align dynamic features in the 3D scans captured by each camera using the nonrigid iterative closest-farthest points algorithm; 2) synchronize scans captured by asynchronous cameras through a novel ADGC-LSTM-based network, which is capable of aligning 3D scans captured by different cameras to the timeline of a specific camera; and 3) register a high-quality template to synchronized scans at each timestamp to form a high-quality 3D mesh model using a non-rigid registration method. With a newly developed 4D foot scanner, we validate the framework and create the first open-access data-set, namely the 4D feet. It includes 4D shapes (15 fps) of the right and left feet of 58 participants (116 feet in total, including 5147 3D frames), covering significant phases of the gait cycle. The results demonstrate the effectiveness of the proposed framework, especially in synchronizing asynchronous 4D scans using the proposed ADGC-LSTM network.

==> Component.tex <==









\begin{tabular}{p{1.2cm} p{2 cm} p{3.5 cm}}%{c c c}%
	\hline\hline
	%& \multicolumn{2}{c}{Component}\\ \cline{2-3}
	Part Number& Description & Application\\
	\hline\hline
	1-6 & Azure Kinect & capturing 3D point cloud \\
	\hline
     7-8 & Mirror &  \\
            \hline
     9 & Glass &  \\
	%\hline
	%9 & ClearVision low-iron glass plate & For capturing sole \\
	%\hline
	%10 & Camera stands & Carrying cameras \\
	%\hline
	%11-12 & Wooden stands & Enough space for user to have three complete steps of walking \\
	\hline\hline
\end{tabular}

==> table_comparision_datasets.tex <==







\begin{tabular}{p{2cm} p{2cm} p{2.6cm} p{3cm} p{3cm} p{1cm}}
	\hline\hline
 Work in & Number of objects & Number of cameras & Speed (fps) - total frames & Time-delay synchronisation & Accuracy (cm)\\
 \hline
 \cite{tajdari2022dynamicregistrationRebuttal} & 3 & 7 (RealSense) & 5 - 15 & Manually & 0.2 \\
 4dcomplete~\cite{li20214dcomplete} & 31 & 1 (unknown) & unknown - 1.972 k & not applicable & 3.74\\
 \cite{boppana2021dynamic} & 30 & 6 (RealSense) & 90 - 1.771 k & Manually & 1 \\
 %\cite{mayer2016large} & 31 & 1 (unknown) & 35000 - unknown & not applicable & 3.74 \\
 SURP~\cite{SUPR:2022} & Not available & 8 (3DMD) & 10 - 1200 k & Manually & 0.9\\
 Ours & 116 & 6 (Azure Kinect) & 15 - 5.147 k & Automatically & 0.68 \\
 %\cite{} & & & & & \\


 

	\hline\hline
\end{tabular}
